Evaluating Transport Protocols on 5G for Mobile Augmented Reality

Mobile Augmented Reality (MAR) mixes physical environments with user-interactive virtual annotations. Immersive MAR experiences are supported by computation-intensive tasks which rely on offloading mechanisms to ease device workloads. However, this introduces additional network traffic which in turn influences the motion-to-photon latency (a determinant of user-perceived quality of experience). Therefore, a proper transport protocol is crucial to minimise transmission latency and ensure sufficient throughput to support MAR performance. Relatedly, 5G, a potential MAR supporting technology, is widely believed to be smarter, faster, and more efficient than its predecessors. However, the suitability and performance of existing transport protocols in MAR in the 5G context has not been explored. Therefore, we present an evaluation of popular transport protocols, including UDP, TCP, MPEG-TS, RTP, and QUIC, with a MAR system on a real-world 5G testbed. We also compare with their 5G performance with LTE and WiFi. Our evaluation results indicate that TCP has the lowest round-trip-time on 5G, with a median of $15.09\pm0.26$ ms, while QUIC appears to perform better on LTE. Through an additional test with varying signal quality (specifically, degrading secondary synchronisation signal reference signal received quality), we discover that protocol performance appears to be significantly impacted by signal quality.

==> unused.tex <==
#Challenges:
1. particular challenges introduced by 5G
2. 

#Related work:
1. https://link.springer.com/content/pdf/10.1007/s11277-017-4999-0.pdf
2. https://www.riverpublishers.com/journal_read_html_article.php?j=JICTS/6/2/8#rfig2
3. https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=5986157
4. https://www.nap.edu/read/4761/chapter/14
(an old paper)
5. https://dl.acm.org/doi/10.1145/3304114.3325616
6. https://tools.ietf.org/html/draft-leiwm-tsvwg-mpmtp-ar-09
7. https://www.w3.org/Mobile/posdep/Oulu.html

**8. https://www.cse.ust.hk/~braudt/papers/PID4718351.pdf  
(Pls carefully check: 
Locating Edge Datacenters for MAR Applications
As justified in the previous sections, the current protocols and the existing architectures cannot provide guarantees in communication delay in the similar way as the classic qual- ity of service guarantees. To handle this problem, network providers have to install edge datacenters close to the users that will be able to handle the MAR offloading requests. Mathematically, this problem can be formulated, in an abstract way, as follows:
minC |C|....
)

#Testbeds to support scalable testing?

#Metrics in evaluation:
1. RTT
2. Throughput
3. Energy consumption on clients (with Mohammad Hoque?)
4. jitter
5. Energy
5, QoE


